Lower Bounds and Improved Algorithms for Asymmetric Streaming Edit Distance and Longest Common Subsequence

In this paper, we study edit distance (ED) and longest common subsequence (LCS) in the asymmetric streaming model, introduced by Saks and Seshadhri [SS13]. As an intermediate model between the random access model and the streaming model, this model allows one to have streaming access to one string and random access to the other string. Our first main contribution is a systematic study of space lower bounds for ED and LCS in the asymmetric streaming model. Previously, there are no explicitly stated results in this context, although some lower bounds about LCS can be inferred from the lower bounds for longest increasing subsequence (LIS) in [SW07][GG10][EJ08]. Yet these bounds only work for large alphabet size. In this paper, we develop several new techniques to handle ED in general and LCS for small alphabet size, thus establishing strong lower bounds for both problems. In particular, our lower bound for ED provides an exponential separation between edit distance and Hamming distance in the asymmetric streaming model. Our lower bounds also extend to LIS and longest non-decreasing sequence (LNS) in the standard streaming model. Together with previous results, our bounds provide an almost complete picture for these two problems. As our second main contribution, we give improved algorithms for ED and LCS in the asymmetric streaming model. For ED, we improve the space complexity of the constant factor approximation algorithms in [FHRS20][CJLZ20] from $\tilde{O}(\frac{n^\delta}{\delta})$ to $O(\frac{d^\delta}{\delta}\;\mathsf{polylog}(n))$, where $n$ is the length of each string and $d$ is the edit distance between the two strings. For LCS, we give the first $1/2+\epsilon$ approximation algorithm with space $n^{\delta}$ for any constant $\delta>0$, over a binary alphabet.

==> asymmetric_ed.tex <==


\section{Asymmetric streaming algorithm for edit distance}

In this section, we presents our space efficient algorithms for approximating edit distance in the asymmetric streaming setting. 

\subsection{Preliminary}

We can compute edit distance exactly with dynamic programming using the following recurrence equation.

\begin{equation}
	\ed(x[1:p], y[1:q]) = \begin{cases}
		\ed(x[1:p-1], y[1:q-1]) , & \text{if $x_p = y_q$.} \\
		\min\begin{cases}
			\ed(x[1:p-1], y[1:q-1])+1, \\
			\ed(x[1:p], y[1:q-1]) + 1, \\
			\ed(x[1:p-1], y[1:q]) + 1, 
		\end{cases}, & \text{if $x_p \neq y_q$.}
	\end{cases}
\end{equation}

Where $ \ed(x[1:p], y[1:q]) $ is the edit distance between $x[1:p]$ and $y[1:q]$.

We can consider a grid graph $G$ whose vertices are nodes on a $(|x|+1)$-by-$ (|y|+1)$ grid, indexed from 0. Horizontal and vertical edges of the form $(i,j)\rightarrow (i+1, j)$ and $(i, j) \rightarrow (i, j+1)$ have weight 1. Diagonal edges of the form $(i,j)\rightarrow (i+1, j+1)$ have weight 0 if $x_i = y_j$ and weight 1 if $x_i \neq y_j$. Then, computing the edit distance between $x$ and $y$ is equivalent to find the shortest path on graph $G$ from vertex $(0,0)$ to vertex $(|x|, |y|)$.



It is equivalent to compute a matrix $A$ dynamically where $A_{p,q}$ equals to $\ed(x[1:p], y[1:q]) $. When the edit distance is bounded by $k$, we only need to compute the diagonal strip of matrix $A$ with width $O(k)$. Thus, we have the following. 

\begin{lemma}[\cite{bibid}]
	\label{lem:O(k)_space_ed}
	Assume we are given streaming access to the online string $x \in \Sigma^*$ and random access to the offline string $y\in \Sigma^n$. Than we can compute $\ed(x,y)$ exactly with $\tilde{O}(\ed(x,y))$ bits of space in $O(n\ed(x,y))$ time. 
\end{lemma}

\begin{claim}
	\label{claim:ed_operation}
	For two strings $x, y\in \Sigma^*$, we can output $\ed(x,y)$ edit operations that transforms $x $ to $y$ with $\tilde{O}(\ed(x,y))$ bits of space in $O(n^2\ed(x,y))$ time. 
\end{claim} 

\begin{proof}
	The idea is to 
\end{proof}

\begin{lemma}
	\label{lem:ed_divide}
	For two strings $x, y \in \Sigma^n$, assume $d = \ed(x,y)$. For any $1\leq t \leq d$, there is a way to divide $x$ and $y$ each into $t$ parts so that $x = x^1\circ x^2 \circ \cdots \circ x^t$ and $y = y^1\circ y^2 \circ \cdots \circ y^t$ (we allow $x^i $or $y^i$ to be empty for some $i$), such that $d = \sum_{i = 1}^t \ed(x^i, y^i)$ and $\ed(x^i, y^i)\leq \lceil\frac{d}{t}\rceil $ for all $i \in [t]$.
\end{lemma}

\begin{proof}
	[Proof of Lemma~\ref{lem:ed_divide}]
	Since $\ed(x,y) = d$, we can find $d$ edit operations on $x$ that transforms $x$ into $y$. We can write these edit operations in the same order as where they occured in $x$. Then, we first find the largest $i_1$ and $j_1$, such that the first $\lceil \frac{d}{t}\rceil$ edit operations transforms $x[1:i_1]$, to $y[1:j_1]$. Notice that $i_1$ (or $j_1$) is 0 if the first $\lceil \frac{d}{t}\rceil$ edit operations insert $\lceil \frac{d}{t}\rceil$ before $x^1$ (or delete first $\lceil \frac{d}{t}\rceil$ symbols in $x$).  We can set $x^1 = x[1:i_1]$ and $y^1 = y[1:j_1]$ and continue doing this until we have seen all $d$ edit operations. This will divide $x$ and $y$ each in to at most $t$ parts. 
\end{proof}



%\begin{lemma}
%	\label{lem:O(k)_space_ed_operations}
%	For two strings $x, y\in \Sigma^*$, we can output $\ed(x,y)$ edit operations that transforms $x $ to $y$ with $\tilde{O}(\ed(x,y))$ bits of space in $O(n^2\ed(x,y))$ time. 
%\end{lemma}

%\subsection{3-approximation algorithm with $\tilde{O}(\sqrt{k})$ space }
%
%% 3-approximation O(\sqrt{k}) space algorithm where a parameter k is given such that k \geq ed
%
%
%\begin{lemma}
%	\label{lem:ed_divide}
%	For two strings $x, y \in \Sigma^n$, assume $d = \ed(x,y)$. There is a way to divide $x$ and $y$ each into $k$ parts so that $x = x^1\circ x^2 \circ \cdots \circ x^t$ and $y = y^1\circ y^2 \circ \cdots \circ y^t$, such that $d = \sum_{i = 1}^t \ed(x^i, y^i)$ and $\ed(x^i, y^i)\leq \lceil\frac{d}{t}\rceil $ for all $i \in [t]$.
%\end{lemma}
%
%\begin{proof}
%	[Proof of Lemma~\ref{lem:ed_divide}]
%	content...
%\end{proof}
%
%Assume an integer $k$ is given to us beforehand such that it is guaranteed $k \leq \ed(x,y)$. We now present our algorithm for approximating $\ed(x,y)$ that uses only $\tilde{O}(\sqrt{k})$ bits of space. The pseudocode is given in Algorithm~\ref{algo:ed_1}. The idea is to utilize Lemma~\ref{lem:ed_divide}. Since we know the edit distance is at most $k$. We can divide $x$ into $O(\sqrt{k})$ blocks and for each block $x^i$, we can find a block in $y$, say $y^i$ such that $\ed(x^i, y^i)$ is at most $\sqrt{k}$.  The purpose of the for-loop starting from line~\ref{algo:ed_1_for1} is to find the longest substring $x^i$ of $x$ starting from position $a_i$, such that, there is a substring of $y$ with edit distance at most $\sqrt{k}$ from $x^i$.   .... triangle inequality....
%
%
%\begin{algorithm}
%	\SetAlgoLined
%	\DontPrintSemicolon
%	\KwIn{Two strings $x, y\in \Sigma^*$ (with streaming access to x), and an upper bound of edit distance $u$}
%	\KwOut{A pair of indices $(p,q)\in [n]\times [n]$ and an integer $l\in n$}
%	\For{ $l' = u - 1$  \textbf{to} $|x|-1$}{\label{algo:longestsubstring_for}
%		try all $1\leq p' <q' \leq n$ such that $l'+1-u \leq |p-q| \leq l'+1+u$. \;
%		compute $\ed(y[p:q], x[1, 1+l'])$. \;	
%		\uIf{exist a pair $p,q$ such that $\ed(y[p:q], x[1, 1+l'])\leq u$}{
%			set $p= p', q = q'$ and $d = \ed(y[p:q], x[1, 1+l'])\leq u$. \;
%			record the edit operations that transform $y[p:q]$ to $x[1, 1+l]$. \;
%			\textbf{continue}
%		}
%		\Else{
%			\textbf{break}
%		}
%		
%	}	
%	\Return{$(p,q)$, $l$, $d$}
%	\caption{LongestSubstring}
%	\label{algo:longestsubsetring}
%\end{algorithm}
%
%
%\begin{algorithm}
%	\SetAlgoLined
%	\DontPrintSemicolon
%	\KwIn{Two strings $x,y\in \Sigma^n$, an integer $k$}
%	\KwOut{An estimation of $\ed(x,y)$ }
%	initialize $i\leftarrow 1$ and $a_i\leftarrow 1$. \;
%	
%	\While{$a_i\leq n$}{
%%		\For{ $j = \sqrt{k} - 1$  to $n-a_i$}{\label{algo:ed_1_for1}
%%			try all $1\leq p <q \leq n$ such that $j+1-\sqrt{k} \leq |p-q| \leq j+1+\sqrt{n}$. \;
%%			compute $\ed(y[p:q], x[a_i, a_i+j])$. \;	
%%			\uIf{exist a pair $p,q$ such that $\ed(y[p:q], x[a_i, a_i+j])\leq \sqrt{k}$}{
%%				set $p_i = p, q_i = q$ and $d_i = \ed(y[p:q], x[a_i, a_i+j])\leq \sqrt{k}$. \;
%%				record the edit operations that transform $y[p:q]$ to $x[a_i, a_i+j]$. \;
%%				\textbf{continue}
%%			}
%%			\Else{
%%				\textbf{break}
%%			}
%%			
%%		}	
%		$(p_i, q_i), l_i, d_i \leftarrow \textbf{LongestSubstring}(x[a_i:n], y, \sqrt{k} )$. \;
%		$ i \leftarrow i+1$.  \;
%		$a_i = a_i + l_i + 1$. \;
%
%	}
%	$T \leftarrow i-1$. \;
%	compute $\tilde{d}$, an $(1+\eps)$-approximation of $\ed(y, y[p_1,q_1]\circ y[p_2, q_2]\circ \cdots \circ y[p_T, q_T])$. \;
%	
%	\Return{$d = \tilde{d} + \sum_{i = 1}^{T}d_i$}\;
%	\caption{$O(\sqrt{k})$ space algorithm}
%	\label{algo:ed_1}	
%\end{algorithm}
%
%
%\begin{lemma}
%	\label{lem:3-approx_ed}
%	Given an integer $k\geq \ed(x,y)$, there is an algorithm that outputs a 3-approximation of $\ed(x,y)$ with $\tilde{O}(\sqrt{k})$ bits of space in polynomial time in the asymmetric streaming model. 
%\end{lemma}
%
%\begin{proof}
%	[Proof of Lemma~\ref{lem:3-approx_ed}]
%	
%\end{proof}
%


\subsection{$2^{O(1/ \delta)}$-approximation algorithm with $\tilde{O}(k^\delta)$ space}


We can futhur reduce the space complexity at the price of a worse but still constant approximation factor. The trade-off is accomplished by using a recursion similar to the algorithm presented by \cite{farhadi2020streaming}.


\begin{algorithm}
	\SetAlgoLined
	\DontPrintSemicolon
	\KwIn{An online $x\in \Sigma^*$ with streaming access, an local string $y\in \Sigma^n$, an upper bound of edit distance $u$, and an upper bound of space available $s$}
	\KwOut{A pair of indices $(p,q)\in [n]\times [n]$, an integer $l\in n$, and an approximation of edit distance $d$}
	\uIf{$u\leq s$}{
		\For{ $l' = u $  \textbf{to} $|x|$}{\label{algo:longestsubstring_for}
			try all $1\leq p' <q' \leq n$ such that $l'-u \leq |q-p+1| \leq l'+u$. \;
			compute $\ed(y[p:q], x[1:l'])$. \;	
			\uIf{exist a pair $p,q$ such that $\ed(y[p:q], x[1: l'])\leq u$}{
				set $p\leftarrow p', q \leftarrow q'$, $d \leftarrow \ed(y[p:q], x[1: l'])\leq u$, and $l \leftarrow l'$. \;
				record the edit operations that transform $y[p:q]$ to $x[1: l']$. \;
				\textbf{continue}
			}
			\Else{
				\textbf{break}
			}
			
		}
	}
	\Else{
		initialize $i = 1$, $a_i = 1$, $l = 0$.  \label{algo:findlongestsubstring_initial}\;
		\While{$a_i\leq |x|$ and $i\leq s$ \label{algo:findlongestsubstring_while}}{
		
			$(p_i, q_i), l_i, d_i \leftarrow \mathsf{FindLongestSubstring}(x[a_i:n], y, \lceil u/s\rceil , s )$. \;
			$ i \leftarrow i+1$.  \;
			$a_i \leftarrow a_{i-1} + l_i $. \;
			$l \leftarrow l+l_i$.\;
		}
		$T \leftarrow i-1$. \;
		for all $1\leq p' < q' \leq n $, compute $\tilde{d}(p',q')$, a $1+\eps$ approxiamtion of $ \ed(y[p':q'], y[p_1:q_1]\circ y[p_2:  q_2]\circ \cdots \circ y[p_T: q_T])$. \;
		$p,q \leftarrow \textbf{argmin}_{p',q'}\tilde{d}(p',q')$.  \Comment*[f]{$p,q$ minimizes $\tilde{d}$}\;
		$d \leftarrow \tilde{d}(p,q)+ \sum_{i = 1}^{T}d_i$. \;
		
		
	}
	\Return{$(p,q)$, $l$, $d$}
	\caption{FindLongestSubstring}
	\label{algo:longestsubstringR}
\end{algorithm}


The main ingredient of our algorithm is a recursive procedure called $\mathsf{FindLongestSubstring}$. The pseudocode is given in algorithm~\ref{algo:longestsubstringR}. It takes four inputs: an online string $x$, an offline string $y$, an upper bound of edit distance $u$, and an upper bound of space available $s$. 

%The goal is to find the largest integer $l$, such that, we can find a substring of $y$, denoted by $y[p:q]$ with $\ed(x[1:l], y[p:q])\leq c u$. 





The output of $\mathsf{FindLongestSubstring}$ consists of three things: a pair of indices $(p,q)$, two integers $l$ and $d$.

\begin{lemma}
	\label{lem:findlongestsubstring}
	Let $(p,q),l, d$ be the output of  $\mathsf{FindLongestSubstring}$ with input $x, y, u, s$. Then assume $l^0$ is the largest integer such that there is a substring of $y$, say $y[p^0: q^0]$, with $\ed(x[1:l^0], y[p^0: q^0])\leq u$. Then, we have $ l\geq l^0$. Also, assume $y[p^*:q^*]$ is the substring of $y$ that is closest to $x[1:l]$ in edit distance. We have 
	\begin{equation}
		\label{eq:findlongestsubstring}
		\ed(x[1:l], y[p^*:q^*]) \leq \ed(x[1:l], y[p':q'])\leq d \leq c(u,v)\ed(x[1:l], y[p^*:q^*]).
	\end{equation}
	Here $c(u,s) = 2^{O(\log_s u)}$ if $u > s$ and $c = 1$ if $ u\leq s$
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:findlongestsubstring}]
	
	In the following, we let $(p,q),l, d$ be the output of  $\mathsf{FindLongestSubstring}$ with input $x, y, u, s$. We let $l^0$ be the largest integer such that there is a substring of $y$, say $y[p^0:q^0]$, with $\ed(x[1:l^0], y[p^0: q^0])\leq u$ and $y[p^*:q^*]$ is the substring of $y $ that minimizes the edit distance to $x[1:l]$
	 
	$\mathsf{FindLongestSubstring}$ first compares $u$ and $s$. If $u\leq s$, we first set $l' = u$, then we know for any $p,q\in [n]$ such that $q-p+1  = u$ , $\ed(x[1:l'], y[p,q])\leq u$ since we can transform $x[1:l']$ to $y[p:q]$ with $u$ substitutions. Thus, we are guaranteed to find such a pair $(p,q)$ and we can record the edit operation that transform $y[p:q]$ to $x[1:l]$. We set $l = l'$, $d = \ed(x[1:l'], y[p:q])$ and continue with $l'\leftarrow l'+1$. When $l'>u$ ($l = l'-1$).  we may not be able to store $x[1:l]$ in the memory for random access since our algorithm uses at most $\tilde{O}(s)$ bits of space. However, we have remembered a pair of indices $(p,q)$ and at most $u$ edit operations that can transform $y[p:q]$ to $x[1:l]$. This allows us to query each bit of $x[1:l]$ from left to right once with $O(u+ l)$ time. Thus, for each substring $y[p:q]$ of y, we can compute its edit distance from $x[1:l']$. Once we find such a substring with $\ed(x[1:l'],y[p:q])\leq u$, we can then compute the edit operations that transfom $y[p,q]$ to $x[1:l']$. Thus, if $u\leq s$, we can find the largest integer $l$ such that there is a substring of $y$, denoted by $y[p:q]$, with $\ed(x[1:l],y[p:q])=u$ with $\tilde{O}(s)$ bits of space. If there is no substring $y[p:q]$ with $\ed(x[1:l'],y[p:q])\leq u$, we terminate the procedure and return current $(p,q)$, $l$, and $d$.
	
	If $l^0> l$, then $x[1:l+1]$ is a substring of $x[1:l^0]$, we can find a substring of $y[p^0:q^0]$ such that its edit distance to $x[1:l+1]$ is at most $u$. Thus, $\mathsf{FindLongestSubstring}$ will not terminate at $l$. We must have $l\geq l^0$.
	
	Also notice that when $u\leq s$, we always do exact computation. $y[p:q]$ is the substring in $y$ that minimizes the edit distance to $x[1:l]$. Thus, Lemma~\ref{lem:findlongestsubstring} is correct when $u\leq s$.
	
	
	For the case $u> s$, $\mathsf{FindLongestSubstring}$ needs to call itself recursively. Notice that each time the algorithm calls itself and enters the next level, the upper bound of edit distance $u$ is reduced by a factor $s$. The recursion ends when $u\leq s$. Thus, we denote the depth of recursion by $d$, where $d = O(\log_s u)$.  We assume the algoirthm starts from level 1 and at level $i$ for $i\leq d$, the upper bound of edit distance is $\frac{u}{s^{i-1}}$. 
	
	
	
	We proof the Lemma by induction on the depth of recursion. The base case of the induction is when $u\leq s$, for which we have shown the correctness of Lemma~\ref{lem:findlongestsubstring}. We now assume Lemma~\ref{lem:findlongestsubstring} holds when the input is $x, y , \lceil u/s\rceil , s$ for any strings $x, y$. 
	
	We first show $l\geq l^0$. Notice that the while loop at line~\ref{algo:findlongestsubstring_while} terminates when either $a_i > |x|$ or $i>s$. If $a_i>|x|$, we know $l$ is set to be $a_i-1  = |x|$. Since $l^0$ is an index of $x$ by definition, $l^0\in [|x|]$. We must have $l\geq l^0$. 
	
	If the while loop terminates when $i>s$. By the definition of $l$, we know $x[1:l^0]$  and $y[p^0: q^0]$ can be divided into $s$ blocks, say, 
	\begin{align*}
		&x[1:l^0] = x[1:l^0_1]\circ x[l^0_1+1:l^0_1 + l^0_2]\circ \cdots \circ x[\sum_{i = 1}^{s-1}l^0_{i}+1:\sum_{i = 1}^{s}l^0_{i}] \\
		&y[p^0:q^0] = y[p^0_1:q^0_1]\circ y[p^0_2:q^0_2]\circ \cdots \circ y[p^0_{s}:q^0_s]
	\end{align*}
	where $l^0 =  \sum_{i = 1}^{s}l^0_{i}$, such that 
	\begin{equation*}
		\ed(x[\sum_{j = 1}^{i-1}l^0_{j}+1:\sum_{j = 1}^{i}l^0_{j}], y[p^0_{i}:q^0_i])\leq \lceil u/s \rceil , \; \forall i\in [s].
	\end{equation*}
	For convenience, we denote $b^0_i = \sum_{j = 1}^{i}l^0_{j}$ and $b_i = \sum_{j = 1}^{i}l_{j}$. By the defintion, we know $b^0_s = l^0$ and $b_s = l$ and all $l^0_i, l_i$ are non-negative. 
	We show that $b_i\geq b^0_i$ for all $i\in [s]$ by induction on $i$. For the base case $i = 1$, let $\bar{l}^0_1$ be the largest such that there is a substring of $y$ within edit distance $\lceil u/s \rceil $ to $x[1: \bar{l}^0_1]$. We know $\bar{l}^0_1 \geq l^0_1$. Since we assume Lemma~\ref{lem:findlongestsubstring} holds for inputs $x, y, \lceil u/s\rceil  , s$, we know $l_1\geq \bar{l}^0_1$. Thus, $l_1\geq l^0_1$ and $b_1\geq b^0_1$. Now assume $b_i\geq b^0_i$ holds for some $i \in [s-1]$, we show that $b_{i+1}\geq b^0_{i+1}$. If $b_i\geq b^0_{i+1}$, $b_{i+1}\geq b^0_{i+1}$ holds. We can assume $ b^0_{i+1} > b_i \geq b^0_{i}$. We show that $l_{i+1}\geq b^0_{i+1}-b_i$. To see this, let $\bar{l}^0_i$ be the largest integer such that there is a substring of $y$ within edit distance $\lceil u/s \rceil$ to $x[b_i+1: b_i+ \bar{l}^0_{i+1}]$. We know $l_{i+1}\geq \bar{l}^0_{i+1}$ since we assume Lemma~\ref{lem:findlongestsubstring} holds for inputs $x[b_i+1:|x|], y, \lceil u/s\rceil  , s$. Notice that $\ed(x[b^0_{i}+1:b^0_{i+1}], y[p^0_i, q^0_i])\leq \lceil u/s\rceil$, we know $\bar{l}^0_i$ is at least $b^0_{i+1}-b_i$ since $x[b_{i}+1:b^0_{i+1}] $ is a substring of $x[b^0_{i}+1:b^0_{i+1}]$. We know $l_{i+1} \geq \bar{l}^0_{i+1}\geq b^0_{i+1}-b_i$. Thus, $b_{i+1} = b_{i}+ l_{i+1}\geq b^0_{i+1}$. This finishes the proof. 
	
	
	
%	When the input is $x, y, u, s$, we first show that $l\geq l^0$. Notice that $x[1:l^0]$ and $y[p^0: q^0]$ can be divided into $s$ parts such that 
%	$$x[1:l^0] = x[l^0_0+1:l^0_1]\circ x[l^0_1+1:l^0_2]\circ \cdots \circ x[l^0_{s-1}+1:l^0_{s}]$$ 
%	$$y[p^0:q^0] = y[p^0_0:q^0_1]\circ y[p^0_1:q^0_2]\circ \cdots \circ y[p^0_{s-1}:q^0_s]$$ 
%	where $l^0_0 = 0$, $l^0_s = l^0$, $p^0_0 = p^0$, $q^0_s = q^0$, and $p^0_i = q^0_i+ 1$ for $1\leq i \leq s-1$, and 
%	$$\ed(x[l^0_{i-1}+ 1:l^0_i], y[p^0_{j-1}:q^0_i])\leq \lceil u/s \rceil , \; \forall i\in [s].$$
	
	%In line~\ref{algo:findlongestsubstring_initial} of algorithm~\ref{algo:longestsubstringR}, we first set $a_1 = 1$ and $i = 1$ and then compute $(p_i, q_i), l_i, d_i$ sequentially. The loop terminates when either $a_i > |x|$ or $i>s$. For the case $a_i\geq |x|$, we have $l = |x|$ which is at least $l^0$. Notice that $a_i = l+1 = |x|+1$. We can divide $ x $ into $i-1$ blocks such that 
	%$$x = x[a_1: a_2-1]\circ x[a_2:a_3-1]\circ \cdots \circ x[a_{i_1}: a_i-1].$$ 
	
	
	
%	Assume $y[p^*:q^*]$ is the substring of $y$ that minimizes edit distance to $x$. We can divide $y[p^*:q^*]$ into $i-1$ parts such that 
%	$$y[p^*:q^*] = y[p^*_1:q^*_1]\circ y[p^*_2:q^*_2]\circ \cdots \circ y[p^*_{i-1}:q^*_{i-1}]$$ 
%	where $p^*_1= p^*$, $q^*_{i-1} = q^*$, and 
%	$$\ed(x[a_j: a_{j+1}-1], y[p^*_{j}:q^*_j])\leq \lceil u/s \rceil , \; \forall j\in [i-1].$$
	
	We now prove inequality~\ref{eq:findlongestsubstring}. After the while loop, the algorithm then finds a substring of $y$, $y[p,q]$, that minimizes $\tilde{d}(p, q)$ where $\tilde{d}(p,q)$ is a $1+\eps$ approximation of $ \ed(y[p':q'], y[p_1:q_1]\circ y[p_2:  q_2]\circ \cdots \circ y[p_T: q_T])$. For convenience, we denote 
	$$\tilde{y} = y[p_1:q_1]\circ y[p_2:  q_2]\circ \cdots \circ y[p_T: q_T]. $$ 
	Thus,
	\begin{equation}
		\label{ed:eq1}
		\ed(y[p:q], \tilde{y}) \leq \tilde{d}(p, q) \leq \tilde{y}(p^*, q^*)\leq   (1+\eps)\ed(y[p^*:q^*], \tilde{y}).
	\end{equation}

	
	Let $y[\bar{p}^*_j: \bar{q}^*_j]$ be the substring of $y$ that is closest to $x[a_j: a_{j+1}-1]$ in edit distance. By the inductive hypothesis, we assume the output of $\mathsf{FindLongestSubstring}(x, y , \lceil u/s \rceil, s)$ satisfies Lemma~\ref{lem:findlongestsubstring}. We know 
	\begin{align}
		\ed(x[a_j: a_{j+1}-1], y[\bar{p}^*_j: \bar{q}^*_j]) &\leq \ed(x[a_j: a_{j+1}-1], y[p_j: q_j]) \notag\\
		&\leq d_j \label{ed:eq2}\\
		&\leq c(u/s,s)\ed(x[a_j: a_{j+1}-1], y[\bar{p}^*_j: \bar{q}^*_j]). \notag
	\end{align}

%	By our assumption that Lemma~\ref{lem:findlongestsubstring} holds when the input is $x, y , \lceil u/s\rceil , s$ for any strings $x, y$. 
	%where $d_j = \ed(x[a_j: a_{j+1}-1], y[p_j: q_j]) $ for $j\in [i-1]$.
	
	By the optimality of $y[p^*:q^*]$ and triangle inequality, we have 

	\begin{align*}
		\ed(x, y[p^*: q^*]) &\leq \ed(x, y[p': q']) & \\
		&\leq \ed(x, \tilde{y}) + \ed( \tilde{y},y[p':q'] ) &\text{By triangle inequality}\\
		& \leq \sum_{i = 1}^{T}d_i + \tilde{d}(p',q') & \\
		& = d & \\
	\end{align*}

	

	Also notice that we can write $y[p^*:q^*] = y[p^*_1: q^*_1]\circ y[p^*_2:q^*_2] \circ \cdots \circ y[p^*_T:q^*_T]$ such that 
	
	\begin{equation}
		\label{ed:eq3}
		 \ed(x[1:l], y[p^*:q^*]) = \sum_{i = 1}^T\ed(x[a_i:a_{i+1}+1], y[p^*_i, q^*_i]).
	\end{equation}
	

	We have
	\begin{align*}
			d & = \sum_{i= 1}^{T}d_j + \tilde{d}(p',q') &\\
%			&\leq \sum_{i= 1}^{T}d_j + \tilde{d}(p^*,q^*) &\\
			& \leq \sum_{i = 1}^{T} d_i + (1+\eps)\ed(\tilde{y}, y[p^*: q^*]) & \text{By \ref{ed:eq1}}\\
			& \leq \sum_{i = 1}^{T} d_i + (1+\eps)\Big(\ed(x[1:l], y[p^*:q^*]) + \ed(x[1:l], \tilde{y})\Big) & \text{By triangle inequality}\\
			&\leq \sum_{i = 1}^{T} d_i + (1+\eps)\sum_{i = 1}^T\ed(x[a_i: a_{i+1}-1], y[p^*_i: q^*_i]) \\
			& \qquad + (1+\eps)\sum_{i = 1}^T\ed(x[a_i:a_{i+1}-1], y[p_i: q_i]) & \\
			& \leq (1+\eps) \sum_{i = 1}^{T} (2c(u/s, s) + 1)\ed(x[a_i: a_{i+1}-1], y[p^*_i: q^*_i]) &\text{By \ref{ed:eq2}} \\
			& \leq (1+\eps)(2c(u/s, s) + 1)\ed(x[1:l], y[p^* : q^*]) & \text{By \ref{ed:eq3}}\\
	\end{align*}
	
	
	We set $c(u, s) = (1+\eps)(2c(u/s, s) + 1)$. Since we assume $c(u/s, s) = O(\log_s u/s)$, we know $c(u,s) = O(\log_s u)$. This proves inequality~\ref{eq:findlongestsubstring}.
	
	
	
	
	
	
	%We know $l_1\geq l^0_1$. We can further show that $\sum_{j = 1}^i \geq l^0$  
	
	%We start from the first position in $x$ and call \mathsf{FindLongestSubstring} with. 
\end{proof}


\begin{lemma}
	\label{lem:findlongestsubstring_space}
	$\mathsf{FindLongestSubstring}(x,y, u, s)$ runs in polynomial time. It queries $x$ from left to right in one pass and uses $\tilde{O}(s\log_s u)$ bits of extra space. 
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:findlongestsubstring_space}]
	If $u\leq s$, we need to store at most $u$ edit operations that transforms, $y[p: q]$ to $x[1:l]$ for current $(p,q)$ and $l$. This takes $\tilde{O}(u) = \tilde{O}(s)$ space. Notice when $l \geq  u$, we do not need to remember $x[1:l]$. Instead, we query $x[1:l]$ by looking at $y[p:q]$ and the edit operations. 

	If $u \geq s $, the algorithm is recursive.  Let us consider the recursion tree. We assume the algoirthm starts from level 1 (root of the tree) and the depth of the recursion tree is $d$. At level $i$ for $i\leq d$, the upper bound of edit distance (third input to algorithm $\mathsf{FindLongestSubstring}$) is $u_i = \frac{u}{s^{i-1}}$. The recursion stops when $u_i\leq s $. Thus, the depth of recursion $d$ is $O(\log_s u)$. The order of computation on the recursion tree is the same as depth-first search and we only need to query $x$ at the bottom level. There are at most $s^d = O(u)$ leaf nodes (nodes at the bottom level). For the $i$-th leaf nodes of the recursion tree, we are computing $\mathsf{FindLongestSubstring}(x[a_i:n], y, u_d, s)$ with $u_d\leq s$ where $a_i$ is the last position visited by the previous leaf node. Thus, we only need to access $x$ from left to right in one pass. 
	
	For each inner node, we need to remember $s$ pairs of indices $(p_i, q_i)$ and $s$ integers $d_i$ for $i\in [s]$, which takes $\tilde{O}(s)$ space. For computing an $(1+\eps)$-approximation of $\tilde{d}(p',q')$, we can use the space-efficient approximation algorithm from~\cite{cheng2020space} that uses only $\polylog(n)$ space. Thus, each inner node takes $\tilde{O}(s)$ bits of space. For the leaf nodes, we have $u\leq s$. Thus, we can compute it with $\tilde{O}(s)$ bits of extra memory. Since the order of computation is the same as depth-first search, we can reuse the space for those nodes we have finished exploring. Thus, total extra space required is $\tilde{O}(s\log_s u)$. This finishes the proof. 


	polynomial time...
\end{proof}



\begin{algorithm}
	\SetAlgoLined
	\DontPrintSemicolon
	\KwIn{Two strings $x,y\in \Sigma^n$, an integer $k$, an upper bound of space $s$}
	\KwOut{An estimation of $\ed(x,y)$ }
	initialize $i\leftarrow 1$ and $a_i\leftarrow 1$. \;
	
	\While{$a_i\leq n$\label{algo:ed_1_loop}}{
		$(p_i, q_i), l_i, d_i \leftarrow \mathsf{FindLongestSubstring}(x[a_i:n], y, k/s, s )$. \;
		$ i \leftarrow i+1$.  \;
		$a_i = a_{i-1} + l_i $. \;
		
	}
	$T \leftarrow i-1$. \;
	compute $\tilde{d}$, an $(1+\eps)$-approximation of $\ed(y, y[p_1:q_1]\circ y[p_2: q_2]\circ \cdots \circ y[p_T: q_T])$. \;
	
	\Return{$d = \tilde{d} + \sum_{i = 1}^{T}d_i$}\;
	\caption{Asymmtric streaming edit distance}
	\label{algo:ed_1}	
\end{algorithm}


\begin{lemma}
	\label{lem:3-approx_ed}
	Given an integer $k\geq \ed(x,y)$, there is an algorithm that outputs a $(3+\eps)$-approximation of $\ed(x,y)$ with $\tilde{O}(\sqrt{k})$ bits of space in polynomial time in the asymmetric streaming model. 
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:3-approx_ed}]
	We run algorithm~\ref{algo:ed_1} with $s = \sqrt{k}$. Since we know $k\geq \ed(x,y)$. We can divide $x$ and $y$ each into $s = \sqrt{k}$ parts such that
	\begin{align*}
		x = x^1\circ x^2 \circ \cdots \circ x^s \\
		y = y^1\circ y^2 \circ \cdots \circ y^s
	\end{align*}
	and $\ed(x^i, y^i)\leq k/s = \sqrt{k}$. We denote $x^i = x[\alpha_i: \beta_i]$ for $i\in [s]$.We have $\alpha_1 = 1$ and $\beta_s = n$.
	
	After running the while loop starting from line~\ref{algo:ed_1_loop}, we get $T$ sets of outputs from $\mathsf{FindLongestSubstring}$, denoted by $(p_j, q_j), l_j, d_j$ for $j\in [T]$. In consistent with the notation in the pseudocode, we have $a_i = \sum_{j = 1}^{i-1}l_{i} + 1$.  Since $k/s = s$, by the analysis of algorithm~\ref{algo:longestsubstringR}, we know $l_i$ is the largest integer such that there is a substring $y[p_i:q_i]$ with $\ed(x[a_i: a_{i}+l_i-1], y[p_i : q_i]) \leq k/s$ for $i\in [T]$. Also, we have $\ed(x[a_i: a_{i}+l_i], y[p_i: q_i])  = d_i$. 
	
	We first show $T\leq s$. Notice that $a_{T+1} = \sum_{i = 1}^{T}l_i +1 = n+1$. We only need to show that $a_{i+1}\geq \beta_i+1$ for $i\in [T]$. This is because if $T>s$, we know $a_{s+1}\geq \beta_s+1 = n+1$, which is contradictory to $a_i\leq n$ when $i\in [T]$. Assume there is some $i\in [T]$ such that $a_{i+1} < \beta_i+1$. Let $i_0 $ be the smallest index such that $a_{i_0+1} < \beta_{i_0}+1$. We know $a_{i_0}\geq \beta_{i_0-1}+1 = \alpha_{i_0}$. We argue that $l_i\geq \beta_{i_0}-\beta_{i_0-1}$. This is because $x[a_{i_0}:\beta_{i_0}]$ is a substring of $x[\alpha_{i_0}, \beta_{i_0}]$. We know $\ed(x^{i_0}, y^{i_0}) = \ed(x[\alpha_{i_0}: \beta_{i_0}], y^{i_0})\leq s$. Therefore, there must exist a susbtring of $y$ whose edit distance to $x[a_{i_0}:\beta_{i_0}]$ is at most $s$. Thus, $l_i\geq \beta_{i_0}-\beta_{i_0-1}$ and $a_{i_0+1} \geq \beta_{i_0}+1$, a contradiction.
	
	Since $T\leq s$, the space used to store $(p_j, q_j), l_j, d_j$ for $j\in [T]$ is $\tilde{s}$. Running $\mathsf{FindLongestSubstring}$ takes a additional $\tilde{s}$ space. 
	
	We now show that $d$ is a $3+\eps$ approximation of $\ed(x,y)$. For convenience, let $\tilde{y} =  y[p_1:q_1]\circ y[p_2: q_2]\circ \cdots \circ y[p_T: q_T]$. Notice that $\ed(x, \tilde{y})\leq \sum_{i = 1}^T \ed(x[a_i: a_{i}+ l_i-1], y[p_i, q_i])$ and $\ed(\tilde{y}, y)\leq \tilde{d}$. 
	We have 
	\begin{align*}
		\ed(x,y) & \leq \ed(x, \tilde{y})+ \ed(\tilde{y}, y) &\text{By triangle inequality}\\
		& \leq \tilde{d} +\sum_{i = 1}^Td_i&\\
		& = d &\\
	\end{align*}
	On the other hand, since we can write $x = x[a_1:a_1+l_1+1]\circ x[a_2:a_2+l_2+1] \circ \cdots \circ x[a_T:a_T+l_T+1]$. We can divide $y$ into $T$ parts such that $y = \hat{y}^1\circ\hat{y}^2 \circ \cdots \circ \hat{y}^T$ and guarantee that 
	\begin{equation*}
		\ed(x, y) = \sum_{i = 1}^T \ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big).
	\end{equation*}
	Also, since $y[p_i:q_i]$ is the substring of $y$ that is closest to $x[a_i:a_i+l_i-1]$ in edit distance, we know
	\begin{equation}
		\label{eq:ed3}
		\ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big) \geq \ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big).
	\end{equation}
	We have
	\begin{align*}
		d & = \tilde{d} +\sum_{i = 1}^Td_i & \\ 
			&\leq (1+\eps) \ed(y, \tilde{y})  + \sum_{i = 1}^T\ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big)  & \\
			& \leq (1+\eps) \Big(\ed(y,x)+ \ed(\tilde{y}, x)\Big)+ \sum_{i = 1}^T\ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big)   & \\
			& \leq (1+\eps) \sum_{i = 1}^T \ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big) + (2+\eps)\sum_{i = 1}^T\ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big)  & \\
			&\leq (3+2\eps) \sum_{i = 1}^T \ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big) & \text{By \ref{ed:eq3}}\\
			&  = (3+2\eps)\ed(x,y).
	\end{align*}

	This shows the output $d$ is indeed a $3+\eps$ approximation of $\ed(x,y)$. 
\end{proof}
 

\begin{lemma}
	\label{lem:2^delta-approx_ed}
	Given an integer $k\geq \ed(x,y)$, for any constant $\delta\in (0,1)$, there is an algorithm that outputs a $2^{O(\frac{1}{\delta})}$-approxiamtion of $\ed(x,y)$ with $\tilde{O}(\frac{k^\delta}{\delta})$ bits of space in polynomial time in the asymmetric streaming model.  
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:2^delta-approx_ed}]
	The proof is similar to the proof of Lemma~\ref{lem:3-approx_ed}. Instead of $s = \sqrt{k}$, we now pick $s = k^\delta$. We can divide $x$ and $y$ each into $s = k^\delta$ parts such that $\ed(x^i, y^i)\leq k/s = k^{1-\delta}$. 

	
	After running the while loop, we get $(p_j, q_j), l_j, d_j$ for $j\in [T]$. We can write $x = x[a_1:a_1+l_1+1]\circ x[a_2:a_2+l_2+1] \circ \cdots \circ x[a_T:a_T+l_T+1]$ and $y$ into $T$ parts such that $y = \hat{y}^1\circ\hat{y}^2 \circ \cdots \circ \hat{y}^T$ and guarantee that 
	\begin{equation*}
		\ed(x, y) = \sum_{i = 1}^T \ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big).
	\end{equation*}

	
	By the same argument as in the proof of Lemma~\ref{lem:3-approx_ed}, we know $T\leq s$ and $\ed(x,y) \leq d$. The space used for running $\mathsf{FindLongestSubstring}$ is, by Lemma~\ref{lem:3-approx_ed}, $\tilde{O}(s\log_s k) = \tilde{O}(k^\delta/\delta)$. We can store $(p_j, q_j), l_j, d_j$ for $j\in [T]$ with an addition $\tilde{O}(k^\delta)$ bits of space and approximate $\ed(y, \tilde{y})$ with $\polylog(n)$ bits of space. The total space used is $\tilde{O}(k^\delta/\delta)$.
	
	By Lemma~\ref{lem:findlongestsubstring}, we know 
	\begin{equation}
		\ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big)\leq c(k, s)\ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big).
	\end{equation}
	Here, $c(k,s) = 2^{O(\log_s k)} = 2^{O(1/\delta)}$. Thus, we can get a similar upper bound of $d$ by
	\begin{align*}
		d & = \tilde{d} +\sum_{i = 1}^Td_i & \\ 
		&\leq (1+\eps) \ed(y, \tilde{y})  + \sum_{i = 1}^T\ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big)  & \\
		& \leq (1+\eps) \Big(\ed(y,x)+ \ed(\tilde{y}, x)\Big)+ \sum_{i = 1}^T\ed\big(x[a_i:a_i+l_i-1], y[p_i: q_i]\big)   & \\
		&\leq (1+\eps)(1+2c(k, k^\delta))\sum_{i = 1}^T \ed\big(x[a_i:a_i+l_i-1], \hat{y}^i\big) & \\
		&  = 2^{O(1/\delta)}\ed(x,y).
	\end{align*}
	
	This finishes the proof. 
\end{proof}

% 2^{O(1/ \delta)} approximation O(k^\delta) algorithm


\subsection{ Using $\tilde{O}(\ed(x,y)^\delta)$ space }

 

\subsubsection{The CGK embedding}

We give a brief introduction to the algorithm presented in \cite{chakraborty2016streaming} that embeds edit distance space into Hamming space. The embedding can be viewed as a function $f: \Sigma^n \times \{0,1\}^l :\rightarrow \Sigma^{3n}$. It takes two inputs: a string $x\in \Sigma^n$ and random bits $r\in  \{0,1\}^l$. $r$ and works as follows. 

We first use $r$ to sample $3n$ random hash functions $h_1,\dots, h_{3n}:\Sigma \rightarrow \{0,1\}$. As is explained in \cite{chakraborty2016streaming}, $l = n(1+\log |\Sigma|)$ is enough for our purpose. At time $t\leq 3n $, we append the symbol $x_i$ to the output. And if $h_t(x_i) = 1$, we increment $i$ by 1. If $i$ exeeds $n$, we pad the output with a fixed symbol $0 \in \Sigma$. 



\begin{lemma}
	\label{lem:cgk_embedding}
	[\cite{chakraborty2016streaming}]
	Given any pair of strings $x,y\in \Sigma^n$ and random bits $r\in \{0,1\}^l$ where $l  = n(1+\log|\Sigma|)$, with probability at least $\frac{2}{3}$, we have
	$$ \frac{1}{2}\ed(x,y)\leq \mathsf{Ham}(f(x,r), f(y,r))\leq O((\ed(x,y))^2).$$
	
	where $\mathsf{Ham}(,)$ denotes the Hamming distance. The probability is over the choice of $r$. 
\end{lemma}

Notice that the embedding can be computed in a streaming way since we only need to read the input string from left to right once. 


\subsubsection{Our algorithm}

 
\begin{algorithm}
	\SetAlgoLined
	\DontPrintSemicolon
	\KwIn{Two strings $x,y\in \Sigma^n$, $\delta \in(0,1)$}
	\KwOut{An estimation of $\ed(x,y)$ }
	initialize $i\leftarrow 1$ and $a_i\leftarrow 1$. \;
	
	set $k$ to to be a large constant and $s = k^\delta$. \;
	\While{$a_i\leq n$}{
		$(p_i, q_i), l_i, d_i \leftarrow \mathsf{FindLongestSubstring}(x[a_i:n], y, k/s, s )$. \label{algo:ed2_findlongestsubstring}\;
		update the approximation of edit distance computed by CGK embedding when we see a new symbol of $x$. Say this value is $\tilde{k}$. When $\tilde{k} \geq k/2$, set $k\leftarrow 4\tilde{k}$ and $s \leftarrow k^\delta$. \label{algo:ed2_cgk}\;  
		$ i \leftarrow i+1$.  \;
		$a_i = a_i + l_i + 1$. \;
		
	}
	$T \leftarrow i-1$. \;
	compute $\tilde{d}$, an $(1+\eps)$-approximation of $\ed(y, y[p_1,q_1]\circ y[p_2, q_2]\circ \cdots \circ y[p_T, q_T])$. \;
	
	\Return{$d = \tilde{d} + \sum_{i = 1}^{T}d_i$}\;
	\caption{Asymmtric streaming edit distance (adaptive $k$)}
	\label{algo:ed_2}	
\end{algorithm}


\begin{lemma}
	\label{lem:2^delta-approx_ed_CGK}
	For any constant $\delta \in (0,1)$, there is a randomized algorithm that computes a $2^{O(1/\delta)}$-approximation of $\ed(x,y)$ in the asymmetric streaming model. With probability at least $2/3$, it uses $\tilde{O}(\frac{1}{\delta}\ed(x,y)^\delta)$ bits of extra space. 
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:2^delta-approx_ed_CGK}]
	For convenience, we use $D$ to denote the actual edit distance between $x$ and $y$. We can iimplement CGK embedding in the asymmetric streaming model with polylog space, assuming we can sample fresh random bits along the computation, to get a $O(D)$-approximation of $D$ with high probability. 
	
	The idea is to run the CGK embedding and algorithm~\ref{algo:ed_1} at the same time. A pseudocode is provided in algorithm~\ref{algo:ed_2}. We note that line~\ref{algo:ed2_cgk} and line~\ref{algo:ed2_findlongestsubstring} are run in parallel. Thus, we update $\tilde{k}$ when ever we read a new symbol of $x$. 
	
	We set $\tilde{k} = 0 $ initially. Notice that CGK embedding maps $x, y\in\Sigma^n$ into $f(x,r), f(y,r)\in \Sigma^{3n}$ using same random bits $r$ and then use $\mathsf{Ham}(f(x,r), f(y,r))$ as an approximation to $\ed(x,y)$. For convenience, we denote $\sigma^x = f(x,r)$ and $\sigma^y = f(y,r)$. We can compute $\sigma^x$ by reading $x$ from left to right once as following. We initially set $\sigma^x$ to be an empty string. When we read an new symbol from $x$, say $x_i$, we append it to $\sigma^x$ $u_i$ times ($u_i$ depends on the randomness $r$). 
	
	Thus, $\sigma^x$ and $\sigma^y$ are of the form
	
	\begin{align*}
		\sigma^x = \underbrace{x_1\dots x_1}_{u_1}\underbrace{x_2\dots x_2}_{u_2}\cdots \underbrace{x_n\dots x_n}_{u_n} \underbrace{0\dots 0}_{3n-\sum_{i = 1}^n u_i },  \\
		\sigma^y = \underbrace{y_1\dots y_1}_{v_1}\underbrace{y_2\dots y_2}_{v_2}\cdots \underbrace{y_n\dots y_n}_{v_n} \underbrace{0 \dots 0}_{3n-\sum_{i = 1}^n v_i }.
	\end{align*}
	
	%That is, in $\sigma^x$ (similar for $\sigma^y$), we repeat the $i$-th symbol of $x$  for some $u_i$ times where $u_i$ is determined by the randomness and then we pad the string with 0's. Here $u_i$ may be different from $v_i$. 
	
	Let $t_i = \sum_{j=1}^{i} u_j$ for $i < n$. Thus, once we have read $x[1:i]$, we can compute $\sigma^x[1:t_i]$. When we read a new symbol $x_i$, we can update $\tilde{k}$ to be $\mathsf{Ham}(\sigma^x[1:t_i], \sigma^y[1:t_i])$ ($\tilde{k}$ before the update is $\mathsf{Ham}\big(\sigma^x[1:t_{i-1}], \sigma^y[1:t_{i-1}]\big)$). Notice that this update can be done in $\polylog(n)$ bits of space by comparing $\sigma^x[t_{i-1}+1:t_i]$ with $\sigma^y[t_{i-1}+1:t_i]$ bit by bit, each bit of $\sigma^y$ can be computed in $\polylog(n)$ bits of space and $\sigma^x[t_{i-1}+1:t_i]$ is just $x_i$ repeated $u_i$ times. 
	
	Let $i'$ be the integer such that $\sum_{j = 1}^{i'-1}v_j < t_i \leq \sum_{j = 1}^{i'}v_j$. We know $\sigma^y_{t_i} = y_{i'}$. Let $\tilde{k}_i = \mathsf{Ham}(\sigma^x[1:t_i], \sigma^y[1:t_i])$. We have $\ed(x[1:i], \ed(y[1:i']))\leq \tilde{k}_i$ for $i<n$. This is because we can build a matching between $x[1:i]$ and $y[1:i']$ such that whenever $\sigma^x_j = \sigma^y_j$ for $j\in [t_i]$, we match the corresponding symbols in $x[1:i]$ and $y[1:i']$. We can transform $x[1:i]$ to $y[1:i']$ with at most $\tilde{k}_i$ edit operations according to the matching.
	
	 We now assume $k$ is updated $u$ times such that $k$ is initially set to be some large constant $k_0$. After the $i$-th update, we denote $k = k_i$. According to our update rule, the update happens whenever $\tilde{k}$ becomes larger than $k/2$ and the updated $k$ is set to be $4\tilde{k}$. Thus, we have $k_i \geq 2k_{i-1}$ for $i\in u$.
	 
	 Let $T_i$ be the number of times we run $\mathsf{FindLongestSubstring}$ with $k = k_i$ so that we have $T = \sum_{i = 0}^u T_i$. We show that $T_i\leq k_i^\delta$. To see this, let $\alpha_i$ be the first position that we run $\mathsf{FindLongestSubstring}$ with input $x[\alpha_i:n], y, k_i^{1-\delta}, k^\delta$. Let $\beta_i$ be the first position that $k_{\beta_i}\geq k_i/2$. Since $\ed(x[1:\beta_i], y[1:\beta'_i])\leq k_{\beta_i}\leq k_i$ for some index $\beta'_i$. We know that there exists a substring of $y$ within edit distance $k_i$ to $x[\alpha_i:\beta_i]$. Also notice that after reading $x_{\beta_i}$, we update $k$ to $k_{i+1}$. By Lemma~\ref{lem:findlongestsubstring}, $T_i\leq    k_i^\delta$. We have 
	 \begin{equation}
	 	T = \sum_{i = 0}^u T_i \leq \sum_{i = 0}^u k_i^\delta \leq k_n^\delta \log k_n
	 \end{equation}
	
	By the correctness of CGK embedding (see Lemma~\ref{lem:cgk_embedding}), we know with probability at least $2/3$, we have $k_n = O(D^2)$. If $k_n = O(D^2)$, we have $T = O(D^{2\delta}\log D)$. Also notice that running $\mathsf{FindLongestSubstring}$ with $k = k_i$ takes an extra $\tilde{O}(k_i^\delta/\delta)$ bits of space. Also, we can compute a $1+\eps$ approximation of $\ed(y, \tilde{y})$ with $\polylog(n)$ space. The extra space required is bounded by $\tilde{O}(D^{3\delta}/\delta)$. 
	
	Notice that we can divide $x$ into $T$ blocks, $x^1, x^2, \dots , x^T$ where $x^i = x[a_i:a_{i+1}-1]$. Let $y^i$ be the substring of $y$ that minimizes $\ed(x^i, y^i)$ for $i\in [T]$. By Lemma~\ref{lem:findlongestsubstring}, we have
	\begin{equation*}
		\ed(x^i, y^i)\leq \ed (x^i, y[p_i, q_i])\leq d_i \leq 2^O(1/\delta)\ed(x^i, y^i).
	\end{equation*}
	The proof of $d$ is a $2^{O(1/\delta)}$ approximation of $D$ is similar to the proof of Lemma~\ref{lem:2^delta-approx_ed}. 
	
	
	
\end{proof}



% combining with CGK embedding, randomized 2^{O(1/ \delta)} approximation O(ed^\delta) algorithm

% CGK embedding




% Then, assume $(p^*,q^*)$ is a pair of indices that minimizes $\ed(x[1:l], y[p^*:q^*])$. We guarantee that $d\leq \ed(x[1:l], y[p:q])\leq c\ed(x[1:l], y[p^*:q^*])$. Here, $c$ is a value determined by $u$ and $s$ which we will calculate later. The algorithm can use at most $\tilde{O}(s)$ bits of extra memory for the computation. 
%
%
%We now explain how it works. \mathsf{FindLongestSubstring} first compares $u$ and $s$. We first set $l' = u$, then we know for any $p,q\in [n]$ such that $q-p+1  = u$ , $\ed(x[1:l'], y[p,q])\leq u$ since we can transform $x[1:l']$ to $y[p:q]$ with $u$ substitutions. Thus, we are guaranteed to find such a pair $(p,q)$ and we can record the edit operation that transform $y[p:q]$ to $x[1:l]$. We set $l = l'$, $d = \ed(x[1:l'], y[p:q])$ and continue with $l'\leftarrow l'+1$. When $l'>u$ ($l = l'-1$).  we may not be able to store $x[1:l]$ in the memory for random access since our algorithm uses at most $\tilde{O}(s)$ bits of space. However, we have remembered a pair of indices $(p,q)$ and at most $u$ edit operations that can transform $y[p:q]$ to $x[1:l]$. This allows us to query each bit of $x[1:l]$ from left to right once with $O(u+ l)$ time. Thus, for each substring $y[p:q]$ of y, we can compute its edit distance from $x[1:l']$. Once we find such a substring with $\ed(x[1:l'],y[p:q])\leq u$, we can then compute the edit operations that transfom $y[p,q]$ to $x[1:l']$. Thus, if $u\leq s$, we can find the largest integer $l$ such that there is a substring of $y$, denoted by $y[p:q]$, with $\ed(x[1:l],y[p:q])=u$ with $\tilde{O}(s)$ bits of space. If there is no substring $y[p:q]$ with $\ed(x[1:l'],y[p:q])\leq u$, we terminate the procedure and return current $(p,q)$, $l$, and $d$.
%
%
%If $u\geq s$, \mathsf{FindLongestSubstring} needs to call itself recursively. We start from the first position in $x$ and call \mathsf{FindLongestSubstring} with space. 


%Say $\bar{l}$ is the largest integer we can find such that there is substring $y[p:q]$ of $y$ with $\ed(x[1:\bar{l}], y[p:q])$.  We start from the first position in $x$ and call \mathsf{FindLongestSubstring} with space 








==> lcs_eps_lower_bound_copy.tex <==
\subsubsection{$\Omega(\frac{r}{\eps})$ lower bound}

We can show a stronger lower bound for $1+\eps$ approximation of $\lcs$ in the asymmetric streaming model. 

\begin{lemma}
	\label{lem:lcs_approx_r_eps}
	Assume $|\Sigma|  = r$, $\eps>0$, and $\frac{r^2}{\eps}  \leq n$ . In the asymmetric streaming model, any deterministic protocol that computes an $1+\eps$ approximation of $\lcs(x,y)$ for any $x, y\in \Sigma^n$, with constant number of passes of $x$ needs $\Omega(\frac{r}{\eps})$ space.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:lcs_approx_r_eps}]
	In the following, we assume the size of alphabet set $\Sigma$ is $3r$ such that 
	$$\Sigma  = \{a_1, b_1, c_1, a_2, b_2, c_2, \dots a_r, b_r, c_r\}. $$
	We let $n_\eps = \Theta(1/\eps)$ such that $n_\eps$ can be divided by 60. 
	
	For any distinct $a,b\in\Sigma$, we can build a set $S_{a,b}$ in the same way as we did in Section~\ref{sec:lcs_exact_det} except that we replace $n$ wtih $n_\eps$ and strings in $S_{a,b}$ are now over alphabet $\{a,b\}$ instead of $\{0,1\}$. Similarly, we can define function $f$ and $\overline{S_{a,b}} = \{f(\sigma) | \sigma\in S_{a,b}\}$. Let $y^{a,b} = a^{n_\eps/3}b^{n_\eps/3} a^{n_\eps/3}$. By Claim~\ref{claim:|S|} and  Lemma~\ref{lem:S}, we know $|S_{a,b}| = |\overline{S_{a,b}}|  = 2^\Omega(n_\eps)$. For any $\sigma\in S_{a,b}$, we have $ \lcs(\sigma\circ f(\sigma), y^{a,b}) = n_\eps/2 + 5$. For any two distinct $\sigma^1, \sigma^2\in S_{a,b}$, we know at least one of $\lcs(\sigma^1\circ f(\sigma^2), y^{a,b})$ and $\lcs(\sigma^2\circ f(\sigma^1), y^{a,b})$ is at larger than $n_\eps/2+5$.
	
	For alphabet $\{a_i, b_i\}$, we can similarly define $S_{a_i, b_i}$, $\overline{S_{a_i, b_i}}$ and  $y^{a_i, b_i}$.  
	
	Consider $w = (w_1, w_2, \dots, w_{2r})$ such that $w_{2i-1} \in S_{a_i,b_i}$ and $w_{2i} \in \overline{S_{a_i,b_i}}$ for $i\in [r]$. Thus, $w$ can be viewed as an element in 
	$$U  =  S_{a_1,b_1}\times \overline{S_{a_1, b_2}}\times \cdots \times S_{a_r,b_r}\times \overline{S_{a_r, b_r}}. $$
	
	%For $i\in [r]$, let $\psi^i(w) = w_{2i-1} \circ w_{2i} \circ c^{10n_\eps}\in\{a,b,c\}^{11n_\eps}$. Then, for any such $w$, we can build a string $\psi(w)\in \{a,b,c\}^{11n_\eps r}$ such that
	
	
	%Thus, $w$ can be viewed as an element in $\underbrace{(S_{a,b}\times \overline{S_{a, b}})\times\cdots \times (S_{a,b}\times \overline{S_{a, b}})}_{r \text{ times}}$. For $i\in [r]$, let $\psi^i(w) = w_{2i-1} \circ w_{2i} \circ c^{10n_\eps}\in\{a,b,c\}^{11n_\eps}$. Then, for any such $w$, we can build a string $\psi(w)\in \{a,b,c\}^{11n_\eps r}$ such that
%	$$\psi(w) = \psi^1(w)\circ \psi^2(w) \circ \cdots \circ \psi^r(w).$$
%	Let $\phi(a,b,c) \in \{a,b,c\}^{11n_\eps r}$ be a string over alphabet $\{a,b,c\}$ such that $\phi(a,b,c)$ is the concatenation of $r$ copies of $a^{n_\eps/3}b^{n_\eps/3}a^{n_\eps/3}c^{10n_\eps}$. Thus 
%	
%	\begin{equation*}
%		\phi =(a^{n_\eps/3}b^{n_\eps/3}a^{n_\eps/3}c^{10n_\eps} )^r.
%	\end{equation*}
%	
%	We write $\phi = \phi(a,b, c)$ when it is clear. 
%	
	Let $\beta = 1/3$. We can define function $h:(S_{a,b}\times \overline{S_{a, b}})^r \rightarrow \{0,1\}$ such that
	\begin{equation}
		h(w) = \begin{cases}
			0, &\text{ if } \forall i\in [r], \;  \lcs(w_{2i-1}\circ w_{2i}, y^{a_i,b_i}) = n_\eps/2 +5 \\
			1, &\text{ if for at least $\beta r$ indices $i\in [r]$, } \lcs(w_{2i-1}\circ w_{2i}, y^{a,b}) > n_\eps/2 +5 .\\
		\end{cases}
	\end{equation}

	
	Consider an error-correcting code $T_{a,b} \subset S_{a,b}^r$ over alphabet $S_{a,b}$ with constant rate $\alpha$ and constant distance $\beta$. We can pick $\alpha = 1/2$ and $\beta = 1/3$ \ref{}, for example. Then the size of the code $T_{a,b}$ is $|T_{a,b} |= |S_{a,b}|^{\alpha r} = 2^{\Omega(n_\eps r)}$.  For any code word $\chi  = \chi_1 \chi_2 \cdots \chi_r \in T_{a,b}$ where $\chi_i\in S_{a,b}$, we can write 
	
	$$\nu (\chi) = (\chi_1, f(\chi_1), \chi_2, f(\chi_2), \dots, \chi_r, f(\chi_r)).$$
	
	In $\chi_i$ and $f(\chi_i)$, we replace alphabet $a, b$ with $a_i, b_i$. 
	
	Let $W = \{\nu(\chi)| \chi\in T_{a,b}\}\in (S_{a,b}\times \overline{S_{a, b}})^r $. Then $|W| = |T_{a,b}| = 2^{\Omega(n_\eps r)}$. We consider a $2r$-player one-way game where the goal is to compute the function $h$ on input $w = (w_1, w_2, \dots, w_{2r})$. In this game, player $i$ holds $w_i$ for $i\in[2r]$ and can only send message to player $i+1$ (Here, $2r+1 = 1$).  We now show the following claim.
	
	\begin{claim}
		\label{claim:W}
		$W$ is a fooling set for the function $h$. 
	\end{claim}

	\begin{proof}
		Consider any two different codewords $\chi, \chi' \in T_{a,b}$. Denote $w = \nu(\chi)$ and $w' = \nu(\chi')$. By our defintion of $w$, we know $w_{2i} = f(w_{2i-1})$ and $w_{2i-1}\in S_{a_i, b_i}$ for $i\in [r]$. We have $\lcs(w_{2i-1}\circ w_{2i}, y^{a_i,b_i}) = n_\eps/2 + 5$. Thus, $h(w) = h(w') = 0$. 
		
		
		The span of $\{w,w'\} $ is the set $\{(v_1, v_2, \dots, v_{2r})| v_i \in \{w_i, w'_i\} \text{ for } i \in [2r]\}$. We need to show that there exists some $v$ in the span of $\{w,w'\} $ such that $h(v) = 1$. Since $\chi, \chi'$ are two different codewords of $T_{a,b}$. We know there are at least $\beta r$ indices $i$ such that $w_{2i-1}\neq w'_{2i-1}$. Let $I\subset [r]$ be the set of indices that $\chi_i\neq \chi'_i$. Then, for $i\in I$, we have 
		\begin{equation*}
			\max\big(\lcs(w_{2i-1}\circ w'_{2i}, y^{a_i,b_i}), \lcs(w'_{2i-1}\circ w_{2i}, y^{a_i,b_i}) )\big) \geq n_\eps + 6. 
		\end{equation*}
		We can build a $v$ as following. For $i\in I$,  if $\lcs(w_{2i-1}\circ w'_{2i}, y^{a,b}\geq n_\eps + 6$. We then set $v_{2i-1} = w_{2i-1}$ and $v_{2i} = w'_{2i}$. Otherwise, we set $v_{2i-1} = w'_{2i-1}$ and $v_{2i} = w_{2i}$. For $i\in [r]\setminus I$, we set $v_{2i-1} = w_{2i-1}$ and $v_{2i} = w_{2i}$. Thus, for at least $\beta r$ indices $i\in [r]$, we have $\lcs(v_{2i-1}\circ v_{2i}, y^{a_i,b_i}) \geq n_\eps/2 +6$. We must have $h(v) = 1$. 
	\end{proof}


	
	Consider a matrix $B$ of size $r\times 2r$ whose rows are elements in $U$. We have  $B_{i,2j-1}\in S_{a_j, b_j}$ and $B_{i, 2j}\in \overline{S_{a_j, b_j}}$. We define the following function $g$. 
	
	\begin{equation}
		g(B) = h(R_1(B))\vee h(R_2(B))\vee \cdots \vee h(R_r(B))
	\end{equation}  
	where $R_i(B)\in U$ is the $i$-th row of matrix $B$ for $i\in [r]$. 
	
	Consider a $2t$ player game where each player holds one column of $B$. The goal is to compute $g(B)$. 
	
	\begin{claim}
		\label{claim:B}
		The set of all $r\times 2r$ matrix $B$ such that $R_i(B)\in U\; \forall\; i\in [r]$ is a fooling set for $g$. 
	\end{claim}
	
	\begin{proof}[Proof of Claim~\ref{claim:B}]
		
	\end{proof}



	We now show how to reduce computing $g(B)$ to approximating the length of LCS in the asymmetric streaming model.
	
	We consider a matrix $\tilde{B}$ of size $r\times (3r+1)$ such that
	\begin{equation}
		\tilde{B}_{i,j} = \begin{cases}
			c_i^{n_\eps}\;, &\text{ if $j\equiv 1 \mod 3$.}\\
			B_{i,\frac{2(j-2)}{3}+1}\;, &\text{ if $j\equiv 2 \mod 3$.}\\
			B_{i,\frac{2(j-3)}{3}+1}\;, &\text{ if $j\equiv 0 \mod 3$.} 
		\end{cases}
	\end{equation}
	$\tB$ is obtained by inserting a column every third position to $B$. The inserted columns are all the same. 
	
	For $j\in [3r+1]$, let $C_j(\tilde{B}) = \tilde{B}_{1,j}\circ  \tilde{B}_{2,j} \circ \dots \circ \tilde{B}_{r,j}$. That is, $C_j(\tilde{B})$ is the concatenation of elements in the $j$-th column of $\tilde{B}$. We can set 
	$$ x  = C_1(\tilde{B})\circ C_2(\tilde{B}) \circ \cdots \circ C_{3r+1}(\tilde{B})\in \Sigma^{(2r+1)rn_\eps }$$
	
	For convenience, let 
	
	$$\phi^i  = c_i^{n_\eps} \circ y^{a_1,b_1} \circ c_i^{n_\eps} \circ y^{a_2,b_2}\circ c_i^{n_\eps} \circ \cdots  \circ c_i^{n_\eps} \circ y^{a_r,b_r} \circ c_i^{n_\eps}\in \Sigma^{(2r+1)n_\eps} .$$ 
	
	We can set
	$$y  = \phi^1\circ \phi^2 \circ \cdots \circ \phi^r \in \Sigma^{11n_\eps r^2} \in \Sigma^{(2r+1)rn_\eps }.$$
	
	Notice that the symbols in different rows of $\tilde{B}$ are different. Symbols in $R_i(\tB)$ can only be matched to $\phi^i$. We can view a longest common subsequence of $x,y$  as a path on matrix $\tB$ from position $(1,1)$ to $(r, 3r+1)$.  So we start from $\tB_{1,1}$ and when some symbol form $\tB_{i,j}$ is picked to the common subsequence, we add $(i,j)$ to the path. Thus, at each step, we can only go down or right.  
	
	We say $j$-th column is a $C$-column if $j\equiv 1 \mod 3$ since elements in $j$-th column of $\tB$ are over alphabet $\{c_1, c_2, \dots, c_r\}$. We argue that the optimal path only goes downward $C$-columns.
	
	To see this, for $j \equiv 1 \mod 3$, $\tB_{i,j}$ has length $n_\eps$. If we go downward on $j$-th column, say from $(i,j)$ to $(i', j)$, we can match all symbols in  $\tB_{i,j}\circ \cdots \circ \tB_{i',j}$. This will give us $(i'-i+1)n_\eps$ matches. 
	
	For $j\not \equiv 1 \mod 3$, $\tB_{i,j}$ has length $n_\eps+5 $ or $n_\eps-5$. Thus, goes through $(i,j)$ for $j\not \equiv 1 \mod 3$ will only add at most $n_\eps+5$ matches. If we go downward on $j$-column. Let $j'>j$ be the smallest integer such that $j' \equiv 1 \mod 3$. Let $(i', j')$ be the first time the path reaches $j'$-th column. Consider an alternative path that first goes right from $(i,j)$ to $(i,j')$ and then goes downward from $(i,j')$ to $(i',j')$. Since each downward step adds at least $n_\eps$ matches, the alternative path gives more matches. 
	
	We now show that $\lcs(x,y)  = \frac{5}{2}n_\eps r + 5 r$ if $ g(B) = 0$ and $\lcs(x,y)\geq \frac{5}{2}n_\eps r + 5 r +  \beta r$  if  $g(B) = 1$.
	
	
	If $g(B) = 0$, we know the optimal path can only go downward on column $j$ when $j\equiv 1 \mod 3$. For $j\equiv 2 \mod 3$, $\tB_{i,j}\circ \tB_{i,j+1}$ can only be matched to $y^{a_{j'}, b_{j'}}$  (Here, $j' = (j+1)/3$) in $\phi^i$. Thus, it can only add $n_\eps/2 + 5$ matches. Since the path goes through $2r$ positions in $C$-columns. Also, for each $j \equiv 2 \mod 3$, it can only go through $(i,j)$ and $(i,j+1)$ in one row. Thus, the size of the match is exactly  $\frac{5}{2}n_\eps r + 5 r$. 
	
	If $g(B) = 1$, there exists some $i\in [r]$ such that $\lcs(R_i(\tilde{B}) , \phi^i)\geq \frac{21}{2}n_\eps r -10 n_\eps +5 r + \beta r$. We then matches all the symbols in $\tB_{1,1}\circ \cdots \circ \tB_{i-1,1}$ (which is a substring of $C_{3r+1}(\tB)$) and all the symbols in $\tB_{1,3r+1}\circ \cdots \circ \tB_{i-1,3r+1}$ (which is a substring of $C_{3r+1}(\tB)$). This gives us a subsequence of $x$ and $y$ of length at least $ \frac{5}{2}n_\eps r + 5 r +  \beta r$. 
	
	Assume $n_\eps = \lambda /\eps$ where $\lambda $ is some constant.  Let $\eps' = \frac{\beta}{10\lambda}$. If we can give a $1+\eps'$ approximation of $\lcs(x,y)$, we can distinguish $g(B) = 0$ and $g(B) = 1$. 



%	\begin{proof}[Proof of Claim~\ref{claim:W}]
%		Consider any two different codewords $\chi, \chi' \in T_{a,b}$. Denote $w = \nu(\chi)$ and $w' = \nu(\chi')$. The span of $\{w,w'\} $ is the set $\{(v_1, v_2, \dots, v_{2r})| v_i \in \{w_i, w'_i\}\}$. We need to show that $h(w) = h(w') = 0$. Also, there exist some $v$ in the span of $\{w,w'\} $ such that $h(v) = 1$.
%		
%		When $w = \nu(\chi)$ for some $\chi\in T_{a,b}$, let us consider the maximum matching between $ \psi(w)$and $\phi$. We first show that one of the best matching between $ \psi(w)$and $\phi$ matches all the $c$ symbols. To see this, we can write $\psi(w)$ and $\phi$ as following
%		\begin{align*}
%			\psi(w) = A_1\circ C_1 \circ A_2 \circ C_2 \circ \cdots \circ A_r \circ C_r \\
%			\phi = A'_1\circ C'_1 \circ A'_2 \circ C'_2 \circ \cdots \circ A'_r \circ C'_r
%		\end{align*}
%		where $A_i, A'_i\in \{a,b\}^{n_\eps}$ and $C_i = C'_i = c^{10n_\eps}$ for $i \in [r]$. Since $A'_j  = y^{a,b} = a^{n_\eps/3}b^{n_\eps/3}a^{n_\eps/3}$ for all $i\in [r]$, we have $\lcs(A_i, A'_j) = n_\eps/2+5$ for all $i, j \in [r]$.
%		
%		We first show that we only need to consider matchings that for any $i$, either no symbols in $C_i$ is mached, or the block $C_i$ is fully matched to some block $C'_j$. To see this, in the matching $m$, let $i$ be the smallest index such that $C_i$ is matched to more than one block in $\phi$. Say $j$ is the smallest index such that some symbol in $C_i$ is matched to $C'_j$. We can build another matching $m'$ that matches every symbol in $C_i $ to $C'_j$ and the remaining are the same as $m$. The size of $m'$ is at least the size of $m$ since the number of matched $c$ symbols will not decrease and the number of matched $a, b$ symbols remains the same. Continue doing this, we get a matching that matches $C_i$ to one block in $\phi$ for all $i\in [r]$.
%		
%		Now, assume the number of unmatched $C$ blocks is $x$. In this case, the number of matched $c$ symbols is $10n_\eps(r-x)$. Since the size of best matching between $A_i$ and $A'_j$ is exactly $n_\eps/2+5$ for any $i, j\in [r]$ and $A$ blocks has length $n_\eps$. One unmatched $C$ block will allow us to match at most $n_\eps /2 -5 $ more $a,b$ symbols. Thus, the best matching always matches all $C$ blocks. We have, 
%		\begin{equation*}
%			\lcs(\psi(w),\phi) = \sum_{i = 1}^r \big(\lcs(A_i, A'_i) + \lcs(C_i, C'_i) \big) = \frac{3}{2}n_\eps r + 5r. 
%		\end{equation*}
%		And thus $h(w) = 0$. 
%		
%		Since $\chi, \chi'$ are two different codewords of $T_{a,b}$. We know there are at least $\beta r$ indices $i$ such that $w_{2i-1}\neq w'_{2i-1}$. Let $I\subset [r]$ be the set of indices that $\chi_i\neq \chi'_i$. Then, for $i\in I$, we have 
%		\begin{equation*}
%			\max\big(\lcs(w_{2i-1}\circ w'_{2i}, y^{a,b}), \lcs(w'_{2i-1}\circ w_{2i}, y^{a,b}) )\big) \geq n_\eps + 6. 
%		\end{equation*}
%		We can build a $v$ as following. For $i\in I$,  if $\lcs(w_{2i-1}\circ w'_{2i}, y^{a,b}\geq \geq n_\eps + 6$. We then set $v_{2i-1} = w_{2i-1}$ and $v_{2i} = w'_{2i}$. Otherwise, we set $v_{2i-1} = w'_{2i-1}$ and $v_{2i} = w_{2i}$. For the remaining $i\in [r]\setminus I$, we set $v_{2i-1} = w_{2i-1}$ and $v_{2i} = w_{2i}$. We have
%		\begin{equation*}
%			h(v) = \lcs(\psi(w),\phi) = \sum_{i = 1}^r \big(\lcs(A_i, A'_i) + \lcs(C_i, C'_i) \big) \geq  \frac{3}{2}n_\eps r + 5r + \beta r. 
%		\end{equation*}
%	
%		Since $v$ is in the span of $w, w'$, we know $ W_{a,b}$ is indeed a fooling for function $h$. 
%		
%		
%	\end{proof}
		
		
		
		
		
		%Consider a matching $m$ between $\psi(w)$ and $\phi$ where not all $c$ symbols are matched. Let $i$ be the smallest integer such that $C_i$ is not fully matched to $C'_i$. There are three cases:
%		
%		\begin{description}
%			\item[Case (1):] Part of $C_i$ is matched to $C'_i$. Without loss of generality, we assume that some symbols in $C_i$ is matched to block $C'_j$ for some $j > i$ (the argument is the same if some symbols in $C'_i$ is matched to block $C_j$ for some $j>i$). Since part of $C_i$ is matched to $C'_i$, block $A_i$ can only be matched to $A'_i$. We consider a different matching $m'$ that is the same as $m$ except $m'$ matches every simbol in block $C_i$ to $C'_i$. This will not change the number of matched $a, b$ symbols. Also, the number of matched $c$ symbols will not decrease. 
%			
%			\item[Case (2):] No symbols in $C'_i$ is matched. 
%			
%			\item[Case (3):] No symbols in $C_i$ is matched. 
%		\end{description}
		
		
		
%		Thus, for any $w\in W_{a, b}$, 
		
		
		
		
		
%		\begin{equation*}
%			%\phi = \underbrace{\underbrace{aa\dots a}_{n_\eps/3 \text{ $a$'s}} \; \underbrace{bb\dots b}_{n_\eps/3 \text{ $b$'s}} \;\underbrace{aa\dots a}_{n_\eps/3 \text{ $a$'s}} \; \underbrace{cc\dots c}_{10n_\eps \text{ $c$'s}}\; \cdots \underbrace{aa\dots a}_{n_\eps/3 \text{ $a$'s}} \; \underbrace{bb\dots b}_{n_\eps/3 \text{ $b$'s}} \;\underbrace{aa\dots a}_{n_\eps/3 \text{ $a$'s}} \; \underbrace{cc\dots c}_{10n_\eps \text{ $c$'s}}}_{\text{$r$ times}}
%%			\phi =\underbrace{ a^{n_\eps/3}b^{n_\eps/3}a^{n_\eps/3}c^{10n_\eps} \cdots a^{n_\eps/3}b^{n_\eps/3}a^{n_\eps/3}c^{10n_\eps}}_{\text{repeated $r$ times}}
%			\phi =(a^{n_\eps/3}b^{n_\eps/3}a^{n_\eps/3}c^{10n_\eps} )^r
%		\end{equation*}
%	
		
	
		
	
	
	
	
	
	
	
	
\end{proof}



